The Regularised Inertial Dean-Kawasaki equation: discontinuous Galerkin approximation and modelling for low-density regime

The Regularised Inertial Dean-Kawasaki model (RIDK) -- introduced by the authors and J. Zimmer in earlier works -- is a nonlinear stochastic PDE capturing fluctuations around the mean-field limit for large-scale particle systems in both particle density and momentum density. We focus on the following two aspects. Firstly, we set up a Discontinuous Galerkin (DG) discretisation scheme for the RIDK model: we provide suitable definitions of numerical fluxes at the interface of the mesh elements which are consistent with the wave-type nature of the RIDK model and grant stability of the simulations, and we quantify the rate of convergence in mean square to the continuous RIDK model. Secondly, we introduce modifications of the RIDK model in order to preserve positivity of the density (such a feature only holds in a ''high-probability sense'' for the original RIDK model). By means of numerical simulations, we show that the modifications lead to physically realistic and positive density profiles. In one case, subject to additional regularity constraints, we also prove positivity. Finally, we present an application of our methodology to a system of diffusing and reacting particles. Our Python code is available in open-source format.

==> extra.tex <==

\section{Potential}

With external potential field $V(\vec x)$,
$$
\frac{\partial\rho}{\partial t}
=-\nabla \cdot \vec{j},\qquad
\frac{\partial \vec{j}}{\partial t}
= -\gamma\,\vec{j} - c\,\nabla\rho + \sigma\,\frac{1}{\sqrt N}\,\sqrt{\rho}\,\vec\xi - \nabla V\,\rho,
$$

With interactive pair potential $W(\vec x)$,

$$
\frac{\partial\rho}{\partial t}
=-\nabla \cdot \vec{j},\qquad
\frac{\partial \vec{j}}{\partial t}
= -\gamma\,\vec{j} - c\,\nabla\rho + \sigma\,\frac{1}{\sqrt N}\,\sqrt{\rho}\,\vec\xi - \rho\,(\nabla W'\star \rho),
$$
\printbibliography 
\end{document}
\section{ Time stepping methods}
For the time discretisation, introduce a time step $\Delta t$ and denote $(\rho_{h,n},j_{h,n})$ as the approximation at time $t_n=n\Delta t$ on $\Omega_h$.
Let $\vec{\xi}_{h,n}\in (S_0)^d$ be an approximation to a sample of the noise $\vec\xi$ at time $t_n$.



 Split-1 (wrt operator $A$)

A:

$$
\begin{aligned}
\rho_t=-\nabla \cdot j, \qquad j_t=-c\nabla \rho.
\end{aligned}
$$

OB:

$$
\begin{aligned}
\rho_t=0,\qquad j_t= -\gamma j - \rho\,(\nabla W \star \rho) - \rho\,\nabla V+\frac{\sigma}{\sqrt N}\sqrt{\rho}\,\xi.
\end{aligned}
$$


Apply A{OB}.

 Split-2 (wrt operator $A$)

A:

$$
\begin{aligned}
\rho_t =-\nabla \cdot j, \qquad j_t=-c\nabla \rho.
\end{aligned}
$$

B:

$$
\begin{aligned}
\rho_t=0,\qquad j_t=  - \rho\,(\nabla W \star \rho) - \rho\,\nabla V.
\end{aligned}
$$

O:
$$
\begin{aligned}
\rho_t=0,\qquad j_t= -\gamma j +\frac{\sigma}{\sqrt N}\sqrt{\rho}\,\xi.
\end{aligned}
$$

Apply BAOAB


 Verlet Splitting

Postion

$$
\begin{aligned}
\rho_t=-\nabla \cdot j, \qquad j_t=0.
\end{aligned}
$$


Velocity:

$$
\begin{aligned}
\rho_t=0,\qquad j_t= -\gamma j- c \,\nabla \rho - \rho\,(\nabla W \star \rho) - \rho\,\nabla V+\frac{\sigma}{\sqrt N}\sqrt{\rho}\,\xi.
\end{aligned}
$$



Each can be integrated exactly over time step $\Delta t$: 

Position:

$$
\begin{aligned}
\rho(t+\Delta t)= \rho(t) -\nabla \cdot j \Delta t.
\end{aligned}
$$





Velocity:

$$
\begin{aligned} \vec j(t+\Delta t) =&e^{-\gamma\, \Delta t} \vec j(t)-\frac{1-e^{-\gamma \Delta t}}{\gamma}(c \,\nabla \rho + \rho\,(\nabla W \star \rho) + \rho\,\nabla V)\\
&+\frac{\sigma}{\sqrt{N}} N(0,\frac{(1-e^{-2\gamma\, \Delta t})}{2\gamma }Q)
\end{aligned}
$$




 BAOAB Splitting

A:
$$
\begin{aligned}
\rho_t=-\nabla \cdot \vec j, \qquad \vec j_t=0.
\end{aligned}
$$
B:
$$
\begin{aligned}
\rho_t=0,\qquad \vec j_t= - c \,\nabla \rho - \rho\,(\nabla W \star \rho) - \rho\,\nabla V.
\end{aligned}
$$
O:
$$
\begin{aligned}
\rho_t=0,\qquad \vec j_t=-\gamma\, \vec j +\frac{\sigma}{\sqrt N}\sqrt{\rho}\,\vec \xi.
\end{aligned}
$$
Each can be integrated exactly over time step $\Delta t$: 

A:
$$\rho(t+\Delta t)= \rho(t) -\nabla \cdot \vec j\, \Delta t.$$

B:
$$\vec j(t+\Delta t)= \vec j(t) -\Big( c \,\nabla \rho + \rho\,(\nabla W \star \rho) + \rho\,\nabla V \Big) \Delta t.$$

O:

$$
\vec j(t+\Delta t) =e^{-\gamma\, \Delta t} \vec j(t)+\frac{\sigma}{\sqrt{N}} N(\vec 0,\frac{(1-e^{-2\gamma\, \Delta t})}{2\gamma }Q)
$$




 \section{Noise}

 (Consider $\xi=\xi_1+\mathrm{i} \,\xi_2$ for independent copies of Federico's $\xi$)


$$
\xi(\vec x)
=\sum_{\vec k}\sqrt{\lambda_{\vec k}} e_{\vec k}(\vec x)\vec \xi_{\vec k}
$$


where each component of $\xi_{\vec k}$ is iid real-valued Gaussian white noise, $e_{\vec k}(\vec x)=e^{\mathrm{i}\,\vec k\cdot \vec x}$ (normalised by $1/\pi^{d}2^{s/2}$ with $s$ is the number of zero modes in dimension $d$).
$\lambda_{\vec  k}=\prod \lambda_{k_i}$, where

$$ 
\lambda_k
= 2\pi \frac{1}{Z_{{\sqrt 2}\epsilon} } e^{-1/2\epsilon^2} I_{|k|} (1/2\epsilon^2).
$$

and $Z_{\sqrt 2 \epsilon}=\int_0^{2\pi} \exp(-\sin^2(y/2)/\epsilon^2))\,dy=2\pi e^{-1/2\epsilon^2} I_0(1/2\epsilon^2)$. Thus,

$$
\lambda_k
=  I_{|k|} (1/2\epsilon^2) / I_0(1/2\epsilon^2).
$$



Note that

$$
Z_{\sqrt 2 \epsilon}=\int_0^{2\pi} \exp (-\frac{\sin^2(x/2)}{\epsilon^2})\,dx.
$$

As $\sin^2(X/2)=\frac 12(1+\cos X)$,
$$
\begin{aligned}
=&
\exp(-1/2\epsilon^2)
 \int_0^{\pi}
\exp(-\frac{\cos(x)} {2\epsilon^2}) 
\cos(jx)\,dx\\
&\quad+
\exp(-1/2\epsilon^2)
 \int_\pi^{2\pi}
\exp(-\frac{\cos(x)} {2\epsilon^2}) 
\cos(jx)\,dx
\end{aligned}
$$


So $\cos(2\pi-x)=\cos(-x)$ and
$\cos(j(2\pi-x))=\cos(-jx)$
$$
\begin{aligned}
=&
\exp(-1/2\epsilon^2)
 \int_0^{\pi}
\exp(-\frac{\cos(x)} {2\epsilon^2}) 
\cos(jx)\,dx\\
&\quad+
\exp(-1/2\epsilon^2)
 \int_0^{\pi}
\exp(-\frac{\cos(x)} {2\epsilon^2}) 
\cos(jx)\,dx
\end{aligned}
$$

Using
$I_j(x)=\frac{1}{\pi}\int_0^\pi \exp(x\cos \theta) \cos(j\theta)\,d\theta$, 
$$
=  \exp(-1/2\epsilon^2) 2\pi I_{j}(1/2\epsilon^2)
$$


Thus, $\lambda_j= Z_{\sqrt 2 \epsilon}^{-1} \,\exp(-1/\epsilon^2) \,2\pi\, I_j(1/2\epsilon^2)$ and
$$
Z_{\sqrt 2 \epsilon}=\,\exp(-1/2\epsilon^2) \,2\pi\, I_0(1/2\epsilon^2)
$$


%  \section{Splitting}

% Consider separately each line. By treating the equations separately, they can be integrated in time. Using splitting technique, this yields an approximation to the full system.

% - Update $\rho$: we seek $\rho_{h,n+1}\in S_k$ such that
% $a(\rho_{h,n+1},\phi)=L(\phi)$
% for all $\phi\in S_k$ with
% $$
% \begin{aligned}
% a(\rho,\phi)
% &=  \int_\Omega  \phi\,\rho  \,dx
% \end{aligned}
% $$

% and
% $$
% \begin{aligned}
% L(\phi)&=\int_\Omega \phi\,\rho_{h,n}
% +\Delta t\, \nabla \phi\cdot \vec j_{h,n}\,d\vec x-\Delta t\sum_\partial 2\{\phi (\vec j_{h,n}\cdot \vec n)\} \int_\partial\,dS.
% \end{aligned}
% $$


% - Update $\vec j$:  by integrating in time, seek $\vec{j}_{h,n+1}\in S_k^d$ such that
% $a(\vec{j}_{h,n+1},\vec\psi)=L(\vec\psi)$
% for all $\vec\psi\in S_k^d$ with
% $$
% \begin{aligned}
% a(\vec j,\vec \psi)
% &= e^{\gamma \Delta t}\int_\Omega \vec \psi\cdot \vec j   \,d\vec x
% \end{aligned}
% $$

% and
% $$
% \begin{aligned}
% L(\psi)&=\int_\Omega \vec \psi\cdot  \vec{j}_{h,n} \,d\vec{x}+\sigma \frac{\Delta t}{\sqrt N}\int_\Omega \sqrt{\rho_{h,n}}\,(\vec\psi\cdot \vec{\xi}_{h,n})\,d\vec{x}\\
% &\quad- \frac{1-e^{-\gamma \Delta t }}{\gamma} c\, 
%  \sum_\partial  2\{\rho_{h,n} (\vec \psi\cdot \vec n)\} \int_\partial\,dS
%  +c \frac{1-e^{-\gamma \Delta t }}{\gamma}
%   \int_\Omega (\nabla\cdot\vec\psi) \rho_{h,n}\,d\vec x.
% \end{aligned}
% $$

% (correction needed for noise term)

